Safe Planning in Interactive Environments via Iterative Policy Updates and Adversarially Robust Conformal Prediction

Safe planning of an autonomous agent in interactive environments -- such as the control of a self-driving vehicle among pedestrians -- poses a major challenge as the behavior of the environment is unknown and reactive to the behavior of the autonomous agent. This coupling gives rise to interaction-driven distribution shifts where the autonomous agent's control policy may change the environment's behavior, thereby invalidating safety guarantees in existing work. Indeed, recent works have used conformal prediction (CP) to generate distribution-free safety guarantees using observed data of the environment. However, CP's assumption on data exchangeability is violated in interactive settings due to a circular dependency where a control policy update changes the environment's behavior, and vice versa. To address this gap, we propose an iterative framework that robustly maintains safety guarantees across policy updates by quantifying the potential impact of a planned policy update on the environment's behavior. We realize this via adversarially robust CP where we perform a regular CP step in each episode using observed data under the current policy, but then transfer safety guarantees across policy updates by analytically adjusting the CP result to account for distribution shifts. This adjustment is performed based on a policy-to-trajectory sensitivity analysis, resulting in a safe, episodic open-loop planner. We further conduct a contraction analysis of the system providing conditions under which both the CP results and the policy updates are guaranteed to converge. We empirically demonstrate these safety and convergence guarantees on a two-dimensional car-pedestrian and a high-dimensional quadcopter case study. To the best of our knowledge, these are the first results that provide valid safety guarantees in such interactive settings.

==> compact_envs_helper.tex <==
% =============================================================
%  compact_envs.tex — INTEGRATION GUIDE
% =============================================================
%  This file documents how to add compact_envs.tex to your
%  existing project. compact_envs.tex itself is STANDALONE and
%  has no dependency on version_toggle.tex or any toggle setup;
%  it works in any LaTeX template.
% =============================================================


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %  WHAT IT GIVES YOU
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  ENV / COMMAND              PRINTS AS
%  ───────────────────────────────────────────────────────────
%  \begin{theoremshort}       **Theorem N (name).** *body*
%  \begin{propositionshort}   **Proposition N (name).** *body*
%  \begin{lemmashort}         **Lemma N (name).** *body*
%  \begin{corollaryshort}     **Corollary N (name).** *body*
%  \begin{definitionshort}    **Definition N (name).** body
%  \begin{assumptionshort}    **Assumption N (name).** body
%  \begin{exampleshort}       **Example N (name).** body
%  \begin{problemshort}       **Problem N (name).** body
%  \begin{remarkshort}        **Remark N (name).** body
%  \sectionshort{T}           **N  T.**  body inline
%  \subsectionshort{T}        **N.M  T.**  body inline
%  \subsubsectionshort{T}     **N.M.K  T.**  body inline
%  \sectionshortstar{T}       **T.**  (no number, no TOC)

%  [name] in brackets is OPTIONAL. Each *short env shares the
%  SAME counter as its full sibling, so numbering is continuous
%  when you mix \begin{theorem} and \begin{theoremshort} in the
%  same paper. \label inside binds to the theorem number; \ref
%  prints that number.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %  INSTALLATION  (ONE LINE in main_toggle.tex)
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  Open main_toggle.tex. Find the THEOREM ENVIRONMENTS block
%  (around the \newtheorem{theorem}{Theorem} declarations).
%  IMMEDIATELY AFTER that block, add:

%    \input{compact_envs}

%  That's it. Your existing \input{version_toggle} continues to
%  work as-is. compact_envs.tex must come AFTER \newtheorem
%  declarations because it references the counters those create.

%  EXAMPLE LOCATION in your main:

%      \newtheorem{theorem}{Theorem}
%      \newtheorem{lemma}{Lemma}
%      \newtheorem{proposition}{Proposition}
%      \newtheorem{corollary}{Corollary}
%      \newtheorem{definition}{Definition}
%      \newtheorem{problem}{Problem}
%      \newtheorem{remark}{Remark}
%      \newtheorem{example}{Example}
%      \newtheorem{assumption}{Assumption}
%      \input{compact_envs}            % <-- ADD THIS LINE

%      \input{version_toggle}          % unchanged, stays where it is


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %  USAGE PATTERNS
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  PATTERN A: same theorem in two forms per build
%  ----------------------------------------------
%  Full block in extended versions (BUILDs 1+2), compact in
%  the short submission (BUILD 3):

%    \begin{fullblock}
%    \begin{theorem}[Safety]\label{thm:safety}
%      The system remains safe for all $t \geq 0$.
%    \end{theorem}
%    \end{fullblock}

%    \begin{shortblock}
%    \begin{theoremshort}[Safety]\label{thm:safety}
%      The system remains safe for all $t \geq 0$.
%    \end{theoremshort}
%    \end{shortblock}

%  \ref{thm:safety} prints the same number in all three builds
%  because both versions step the SAME `theorem' counter.


%  PATTERN B: same section heading, full vs run-in per build
%  ----------------------------------------------------------
%    \begin{fullblock}
%    \section{Problem Formulation}\label{sec:problem}
%    \end{fullblock}
%    \begin{shortblock}
%    \sectionshort{Problem Formulation}\label{sec:problem}
%    \end{shortblock}

%    We consider a discrete-time dynamical system ...


%  PATTERN C: in a generic template (no toggles at all)
%  ----------------------------------------------------
%  compact_envs.tex works without any toggle infrastructure:

%    \documentclass{article}
%    \usepackage{amsthm}
%    \newtheorem{theorem}{Theorem}
%    \newtheorem{lemma}{Lemma}
%    \input{compact_envs}
%    \begin{document}

%    \begin{lemmashort}[Continuity]
%    The map $f$ is continuous.
%    \end{lemmashort}

%    \end{document}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %  CUSTOMIZATION
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  Adding a new short env: one line in compact_envs.tex.

%    \newshorttheorem{conjectureshort}{Conjecture}{conjecture}{\itshape}
%                        ^^^env name^^   ^display^   ^counter^   ^style^

%  Make sure \newtheorem{conjecture}{Conjecture} is declared in
%  main_toggle.tex first.

%  Removing a short env: comment out its \newshorttheorem line.
%  The corresponding full theorem env still works.

%  Tightening vertical space: in compact_envs.tex, change the
%  closing argument of the factory from \par\medskip to
%  \par\smallskip or just \par.

%  Switching style of an existing env: change the \itshape /
%  \upshape argument on its \newshorttheorem line.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %  TROUBLESHOOTING
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  ERROR: "No counter `theorem' defined."
%    CAUSE: \input{compact_envs} ran BEFORE
%           \newtheorem{theorem}{Theorem}.
%    FIX:   Move \input{compact_envs} to AFTER the \newtheorem
%           block.

%  ERROR: "No counter `problem' defined." (or any other counter)
%    CAUSE: compact_envs.tex declares a *short variant for a
%           counter you haven't created. E.g., problemshort needs
%           \newtheorem{problem}{Problem}.
%    FIX:   Either declare the missing \newtheorem in your main,
%           or comment out the matching \newshorttheorem line in
%           compact_envs.tex.

%  ERROR: "Environment theoremshort undefined."
%    CAUSE: compact_envs.tex did not load (typo in \input,
%           file in wrong directory, or earlier compile error
%           aborted before reaching \input{compact_envs}).
%    FIX:   Verify the file is at the path \input expects, and
%           that there are no earlier compile errors.

%  NUMBERING JUMPS UNEXPECTEDLY:
%    CAUSE: You have a \begin{theorem} inside a fullblock and a
%           \begin{theoremshort} inside a shortblock for the
%           same statement, but the labels point to different
%           numbers in different builds.
%    FIX:   Both versions step the SAME counter, so this should
%           not happen. If it does, check whether you accidentally
%           declared theoremshort with a different counter (the
%           3rd argument of \newshorttheorem).


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %  WHAT THIS FILE DELIBERATELY DOES NOT DO
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  - It does NOT touch your version_toggle.tex.
%  - It does NOT define any toggle commands.
%  - It does NOT depend on \iffullcontent, \ifarticleclass, etc.
%  - It does NOT load amsthm, jmlrutils, or any other package.
%  - It does NOT redefine \section, \subsection, \subsubsection.
%    The compact \sectionshort etc. coexist with normal \section.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> compact_math.tex <==
% =============================================================
% compact_math.tex  --  TIGHTER VERTICAL SPACING AROUND DISPLAY MATH
% =============================================================
% A drop-in helper file that tightens the vertical glue around
% every display-math block (\begin{equation}, \begin{align},
% \begin{align*}, \begin{gather}, \[ ... \], etc.) and the line
% spacing inside align/gather. Completely STANDALONE: no
% dependency on version_toggle.tex, on any \if-flag, or on any
% document class.
%
% USE WITH ANY TEMPLATE / ANY VERSION / ANY TOGGLE SETUP.
% =============================================================
%
% USAGE: in your main file, at any point in the preamble, add:
%
%   \input{compact_math}
%
% That's it. The tightening applies automatically to EVERY
% display equation in the document, in every build.
%
% =============================================================
% IMPLEMENTATION NOTE  (why \AtBeginDocument is required)
% =============================================================
% The five lengths below are font-size-dependent and are
% reset by \normalsize, which is called by \begin{document}.
% Setting them in the preamble naively does nothing: the
% reset overwrites your values. The correct hook is
% \AtBeginDocument{...}, which fires AFTER \normalsize has
% initialized.
%
% This file uses that hook automatically. Override the values
% (in the preamble or after \input{compact_math}) by changing
% the \setlength lines below — your values will then be the
% ones applied at \begin{document}.
% =============================================================
%
% =============================================================
% TUNABLE LENGTHS
% =============================================================
%
%   \compactabovedisplay        space ABOVE display math (long-line case)
%   \compactbelowdisplay        space BELOW display math
%   \compactaboveshortdisplay   space ABOVE when preceded by short line
%   \compactbelowshortdisplay   space BELOW when above-short was used
%   \compactjot                 vertical space between lines in align/gather
%
% Defaults are set below. Override in your preamble:
%
%   \setlength{\compactabovedisplay}{4pt plus 1pt minus 1pt}
%   \setlength{\compactbelowdisplay}{4pt plus 1pt minus 1pt}
%   \setlength{\compactaboveshortdisplay}{0pt plus 1pt}
%   \setlength{\compactbelowshortdisplay}{4pt plus 1pt minus 1pt}
%   \setlength{\compactjot}{2pt}
%
% =============================================================
% REFERENCE: STANDARD DEFAULTS
% =============================================================
%
% --- ARTICLE / JMLR / L4DC at 10pt -----------------------
%   \abovedisplayskip        10pt plus 2pt minus 5pt
%   \belowdisplayskip        10pt plus 2pt minus 5pt
%   \abovedisplayshortskip    0pt plus 3pt
%   \belowdisplayshortskip    6pt plus 3pt minus 3pt
%   \jot                      3pt
%
% --- ARTICLE / JMLR / L4DC at 11pt -----------------------
%   \abovedisplayskip        11pt plus 3pt minus 6pt
%   \belowdisplayskip        11pt plus 3pt minus 6pt
%   \abovedisplayshortskip    0pt plus 3pt
%   \belowdisplayshortskip    6.5pt plus 3.5pt minus 3pt
%   \jot                      3pt
%
% --- DEFAULTS CHOSEN HERE --------------------------------
%   \compactabovedisplay         4pt plus 1pt minus 1pt
%   \compactbelowdisplay         4pt plus 1pt minus 1pt
%   \compactaboveshortdisplay    0pt plus 1pt
%   \compactbelowshortdisplay    4pt plus 1pt minus 1pt
%   \compactjot                  2pt
%
% Net per display equation: ~12pt vertical space reclaimed
% relative to the 10pt class default. For a paper with ~30
% display equations, this is roughly 360pt ~ 27 lines ~ 0.7
% columns reclaimed AUTOMATICALLY across the whole document.
%
% =============================================================
% ILLUSTRATIVE EXAMPLES
% =============================================================
% Below, "x" is body text, "===" represents the equation,
% blank lines represent vertical glue. Each example shows the
% same source (one paragraph of text -> equation -> next
% paragraph of text) rendered with different settings.
%
% --- A. STOCK 10pt CLASS (no compact_math.tex loaded) ---
% \abovedisplayskip = \belowdisplayskip = 10pt
%
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%
%
%             ============= eq =============
%
%
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%
% Total whitespace around equation: ~20pt
%
% --- B. DEFAULTS IN THIS FILE (4pt above, 4pt below) ---
%
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%
%             ============= eq =============
%
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%
% Total whitespace: ~8pt   (saves ~12pt per equation)
%
% --- C. AGGRESSIVE (2pt above, 2pt below) ---
% Override:
%   \setlength{\compactabovedisplay}{2pt plus 1pt}
%   \setlength{\compactbelowdisplay}{2pt plus 1pt}
%
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%             ============= eq =============
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%
% Total whitespace: ~4pt   (saves ~16pt per equation)
%
% --- D. ZERO (extreme; only for desperate cases) ---
% Override:
%   \setlength{\compactabovedisplay}{0pt}
%   \setlength{\compactbelowdisplay}{0pt}
%
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%             ============= eq =============
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%
% Total whitespace: 0pt    (saves ~20pt per equation, but math
%                           collides visually with text;
%                           usually unacceptable)
%
% --- E. ASYMMETRIC (3pt above, 5pt below) ---
% Useful when the eq introduces a new clause that needs
% breathing room AFTER it more than before:
%   \setlength{\compactabovedisplay}{3pt plus 1pt}
%   \setlength{\compactbelowdisplay}{5pt plus 1pt minus 1pt}
%
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%
%             ============= eq =============
%
%
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%   xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%
% --- F. \jot EXAMPLE (multi-line align) ---
% Default \jot=3pt vs compact_math default \jot=2pt vs aggressive 0pt:
%
% \jot=3pt (stock):                 \jot=2pt (default):           \jot=0pt:
%   line 1 of align              line 1 of align              line 1 of align
%                                                            line 2 of align
%   line 2 of align              line 2 of align              line 3 of align
%                                line 3 of align
%   line 3 of align
%
% Per-paper impact for a 5-line align: 8pt -> 4pt -> 0pt savings.
% =============================================================
%
% ADVICE ON TUNING
% =============================================================
% Try defaults first. If page count is fine but math feels
% cramped, loosen to 6pt+6pt. If still over budget, tighten to
% 2pt+2pt. Avoid 0pt unless the alternative is being rejected
% for length.
% =============================================================

% --- Double-load guard (safe to \input multiple times) ---
\expandafter\ifx\csname compactmathloaded\endcsname\relax\else\endinput\fi
\expandafter\let\csname compactmathloaded\endcsname\empty

% --- Tunable spacing lengths -----------------------------
\newlength{\compactabovedisplay}
\setlength{\compactabovedisplay}{4pt plus 1pt minus 1pt}

\newlength{\compactbelowdisplay}
\setlength{\compactbelowdisplay}{4pt plus 1pt minus 1pt}

\newlength{\compactaboveshortdisplay}
\setlength{\compactaboveshortdisplay}{0pt plus 1pt}

\newlength{\compactbelowshortdisplay}
\setlength{\compactbelowshortdisplay}{4pt plus 1pt minus 1pt}

\newlength{\compactjot}
\setlength{\compactjot}{2pt}

% --- Apply the lengths AFTER \normalsize has initialized ---
% This is the critical part: \begin{document} calls
% \normalsize which resets the four display-skip lengths
% from the class's font tables. We hook AFTER that so our
% values become the ones that stick.
\AtBeginDocument{%
  \setlength{\abovedisplayskip}      {\compactabovedisplay}%
  \setlength{\belowdisplayskip}      {\compactbelowdisplay}%
  \setlength{\abovedisplayshortskip} {\compactaboveshortdisplay}%
  \setlength{\belowdisplayshortskip} {\compactbelowshortdisplay}%
  \setlength{\jot}                   {\compactjot}%
}


==> sections/04_case_study_car_pedestrian.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.35\linewidth]{figure/1}
    \includegraphics[width=0.36\linewidth]{figure/2}\\
    \includegraphics[width=0.35\linewidth]{figure/3}
    \includegraphics[width=0.35\linewidth]{figure/4}
    \caption{Two-dimensional car--pedestrian case study. Top left: evolution of the planning radius $r_j$ over episodes. Top right: evolution of the optimal cost $J_j$. Bottom left: empirical tube coverage $\mathbb{P}\{y_{j,0:T}\in \mathcal{C}_{r_j}(\hat y_{0:T})\}$. Bottom right: empirical safety coverage $\mathbb{P}\{H(x_{j,0:T},y_{j,0:T})\le 0\}$.}
    \label{eq:results}
\end{figure}

\subsection{Case Studies}
\label{sec:case_studies}

\section{2D Car--Pedestrian Interaction}
\label{sec:ped-main}

\subsubsection{Model and Planning Setup}

We instantiate the running vehicle--pedestrian example in two dimensions. The ego car state is $x_t\in \mathbb{R}^2$ and evolves according to the single-integrator dynamics $x_{t+1}=x_t+\Delta u_t$ with sampling time $\Delta:=0.1$ and component-wise control bound $\|u_t\|_\infty \le u_{\max}:=2$. The pedestrian state is $y_t\in \mathbb{R}^2$ and evolves according to the interactive dynamics
\begin{align*}
    y_{t+1} = y_t + \Delta\big(v_0 + \phi(\|r_t\|_2)e_t\big) + w_t,
\end{align*}
where $r_t := y_t - x_t$ is the relative position, $e_t:=r_t/\|r_t\|_2$ is the normalized relative position, $v_0:=\begin{bmatrix} -0.5 & 0\end{bmatrix}^T$ is the nominal velocity, and $w_t \sim \mathcal{N}(0, \Delta \sigma^2 I)$ with $\sigma:=0.05$. The interaction function
\[
\phi(\|r_t\|_2) := v_{\max} \frac{\ell_c^2}{\|r_t\|_2^2 + \ell_c^2}
\]
models a repulsive effect with maximum speed $v_{\max}:=1$ and interaction distance $\ell_c:=1$. Importantly, the predictor available to the planner does not know this interaction law; it uses the nominal model
\[
\hat y_{t+1}=\hat y_t+\Delta v_0,
\qquad
\hat y_0:=y_0:= \begin{bmatrix} 3 & 1.5 \end{bmatrix}^T.
\]

The planner minimizes
\begin{align*}
    J(x,u):= w_{\text{goal}} \|x_{T} - x_{\text{goal}}\|_2^2 + w_{\text{track}} \sum_{t=0}^{T-1} \|u_t\|_2^2
\end{align*}
with goal $x_{\text{goal}}:=\begin{bmatrix} 6 & 0.5\end{bmatrix}^T$, weights $w_{\text{goal}}:=1$ and $w_{\text{track}}:=0.0001$, and horizon $T:=50$ (that is, $T\Delta=5$ seconds). Safety is encoded by
\[
H(x,y):=\max_{0\le t\le T}\big(d_{\min} - \|x_t - y_t\|_2\big),
\]
where $d_{\min}:=0.8$ is the required minimum separation. Throughout this case study we use $\alpha:=0.1$, $\delta:=0.05$, and $n_j:=1000$ rollout trajectories for each recalibration step.

\subsubsection{Simulation Protocol and Implementation Details}
\label{subsec:ped-sim-protocol}

At episode $j$, given a planning radius $r_j$, we compute the ego policy $\pi_j=\pi^\star(r_j)$ by solving the robust program $\mathbf{P}[j;\,r_j]$ in~\eqref{eq:episodic}. For the Euclidean tube in this case study, robust satisfaction of $H(x,\zeta)\le 0$ for all $\zeta\in\mathcal{C}_{r_j}(\hat y_{0:T})$ is enforced through the deterministic tightening
\[
\|x_{j,t}-\hat y_t\|_2 \ \ge\ d_{\min}+r_j,
\qquad t=0,\ldots,T,
\]
which follows directly from the triangle inequality and the tube definition in~\eqref{eq:score-tube}. The resulting finite-dimensional nonlinear program is solved in MATLAB using \texttt{fmincon}, warm-started with the previous episode's solution.

After deploying $\pi_j$, we collect $n_j$ i.i.d. interactive rollouts $\{y^{(i)}_{j,0:T}\}_{i=1}^{n_j}\sim\mathcal{D}(\pi_j)$ and compute the nonconformity scores from~\eqref{eq:score-tube}. We then form the per-episode quantile $q_j$ via~\eqref{eq:episodic_quantile}. The theory and appendices support both the implicit and explicit transfer rules; the quantitative results in Figure~\ref{eq:results} use the explicit update with fixed sensitivity constants, while Appendix~\ref{sec:iterative_algorithm} records the implementation-level pseudocode for both solver realizations.

\subsubsection{Observed Behavior}

Figure~\ref{eq:results} reports the radius $r_j$, the optimal cost $J_j$, the empirical tube coverage $\mathbb{P}\{y_{j,0:T}\in \mathcal{C}_{r_j}\}$, and the empirical safety coverage $\mathbb{P}\{H(x_{j,0:T},y_{j,0:T})\le 0\}$ across episodes. The main qualitative picture is consistent with the theory developed in Section~\ref{sec:analysis}. The radius contracts rapidly from its conservative initialization and then stabilizes, the cost improves accordingly as the planner becomes less conservative, and both the tube coverage and the safety coverage remain near their intended levels.

This example is important because the predictor is intentionally misspecified: the planner only sees the nominal pedestrian model, while the deployed pedestrian reacts to the ego policy through the repulsive interaction law. The iterative loop therefore has to do two jobs simultaneously: learn how conservative the safety tube should be under the current policy, and protect the next policy against the shift that its own update may induce. The fact that the radius, performance, and empirical safety all stabilize together is the main empirical validation of the theory-facing pipeline. Section~\ref{sec:quadswarm} then isolates the effect of the baseline construction and the radius-update rule in a more homogeneous multi-agent setting.


==> sections/05_case_study_quadswarm_homogeneous.tex <==
\subsection{Ablation Study: Multi-Quadcopter Navigation in a Homogeneous Interactive Swarm}
\label{sec:quadswarm}

We next study a more homogeneous interaction pattern in a multi-quadcopter navigation task built on the open-source QuadSwarm simulator~\cite{quadswarm}. The role of this experiment is different from the vehicle--pedestrian case study: here the goal is to isolate the effect of the radius-update rule itself. Because all agents are trained with similar collision-averse navigation objectives, the induced policy-dependent shift is milder and more homogeneous. As a result, the experiment cleanly separates two questions: which update rules remain conservative, and which ones actually convert that conservatism into additional reward.

\subsection{Environment, Interaction Mechanism, and Safety Filtering}
\label{sec:quadswarm-env}

We consider one ego quadrotor and $N_{\mathrm{env}}=5$ environment quadrotors (six agents total). At the planning layer, each agent is modeled as a double integrator in $\mathbb{R}^3$, so the task fits the coupled formulation in~\eqref{eq:pf:dyn}. Interaction arises because the environment agents are controlled by learned navigation policies trained with collision penalties: proximity to other quadrotors, including the ego, is penalized during training, which makes their closed-loop behavior reactive to the ego motion. The environment agents do not use a hard safety filter at test time, so collision avoidance is encouraged by the reward but not guaranteed by a separate controller.

Safety is enforced only on the ego. Concretely, the ego deploys a CBF-QP safety filter around a fixed, pre-trained RL policy. To align with the episodic notation in~\eqref{eq:episodic}, we write the deployed ego policy in episode $j$ as
\begin{equation}
\pi_j := \mathrm{CBF\mbox{-}QP}(\pi^{\mathrm{RL}},\,r_j),
\label{eq:quadswarm-deployed-policy}
\end{equation}
where the learned nominal policy $\pi^{\mathrm{RL}}$ is fixed, and the deployed policy changes only through the radius $r_j$. A collision is declared whenever an inter-agent distance falls below $d_{\mathrm{coll}}:=2.5\,\ell_{\mathrm{arm}}$, where $\ell_{\mathrm{arm}}$ is the quadrotor arm length in the simulator.

\subsection{Reference Predictor, Baselines, and Update Protocol}
\label{sec:quadswarm-loop}

We use the trajectory score in~\eqref{eq:score-tube} with the Euclidean norm in $\mathbb{R}^3$. For each episode $j$, we collect $n_{\mathrm{cal}}=200$ interactive rollouts under the deployed policy $\pi_j$ and compute per-agent empirical quantiles of the trajectory score. Because safety must hold simultaneously with respect to all $N_{\mathrm{env}}$ environment quadrotors, we aggregate them through a single interactive quantile $\hat q_j:=\max_i q_j^{(i)}$. The admissible radius set is $\mathcal{R}=[r_{\min},r_{\max}]$ with $r_{\min}=2\,\ell_{\mathrm{arm}}$ and $r_{\max}=8\,\mathrm{m}$, and the explicit transfer update uses $\kappa=0.6$.

All four compared methods use the same conservative initialization $r_0=r_{\max}$ and the same homogeneous reference predictor $\hat y_{0:T}^{\mathrm{ref}}$, obtained from a rollout in which the ego follows the same nominal navigation policy as the environment agents. This choice provides a neutral reference trajectory consistent with the homogeneous training distribution.

The baselines differ only in how they treat recalibration and transfer after the first rollout-induced certificate is computed:
\begin{itemize}
    \item \emph{Robust (ours):} after every episode, recalibrate on the newly collected interactive data and update the next radius through the transfer recursion~\eqref{eq:r_update}. Because the initialization is conservative, the first explicit update shrinks from $r_0=8\,\mathrm{m}$ to approximately $3.82\,\mathrm{m}$ rather than jumping directly to the first quantile.
    \item \emph{Naive:} recalibrate each episode but drop the transfer term, so the next radius is set directly to the freshly measured quantile. In the displayed run this means $r_1\approx q_0\approx1.31\,\mathrm{m}$ and $r_2\approx q_1\approx1.07\,\mathrm{m}$.
    \item \emph{Calibrate-once:} reuse the first calibrated certificate throughout the displayed episode window. In the uploaded plots this produces a fixed radius near $1.31\,\mathrm{m}$ over the first ten episodes.
    \item \emph{Non-interactive:} keep the same first calibrated radius without any transfer logic. In the current homogeneous plots, this curve is numerically almost indistinguishable from the calibrate-once baseline over the displayed horizon because both inherit the same initial certificate.
\end{itemize}
For reporting, we generate an additional 100 rollouts per episode to estimate empirical tube coverage, empirical safety coverage, and cumulative progress-to-goal reward.

\subsection{Results and Interpretation}
\label{sec:quadswarm-results}

Figure~\ref{fig:quadswarm-metrics} summarizes the quantitative behavior. The proposed robust update contracts the radius rapidly from the conservative initialization and stabilizes near $1\,\mathrm{m}$ within the first few episodes (for example, $r_1\approx 3.82\,\mathrm{m}$ and $r_5\approx 1.02\,\mathrm{m}$). This contraction is accompanied by a clear reward increase, from roughly $1.6$ in the first displayed episode to about $2.68$ once the radius stabilizes. Empirical tube coverage stays at or above the target $1-\alpha=0.9$, and empirical safety coverage remains one in the reported rollouts.

The main question in this homogeneous setting is why the baselines do not fail dramatically. The reason is that the environment agents already expect collision-averse behavior from their training distribution, and the homogeneous reference predictor remains close to the realized trajectories even when the ego policy changes moderately. Consequently, the no-transfer \emph{naive} baseline does not oscillate: once it jumps directly to the observed quantile, the subsequent quantiles change only mildly. Nevertheless, it remains slightly more conservative than the robust update and attains slightly lower reward. In other words, removing transfer is not catastrophic here, but it still leaves performance on the table.

The fixed-radius baselines tell a different story. Over the displayed episode window, the \emph{calibrate-once} and \emph{non-interactive} curves are nearly identical because both reuse the same first certificate. This should not be interpreted as evidence that transfer is unnecessary. Rather, in this particular homogeneous regime the first certificate is already reasonably aligned with the deployed distribution, so the principal effect of continued updating is not safety recovery but conservatism reduction. That is why all methods achieve empirical safety close to one, while the robust method is still the most rewarding: it is the only method that systematically converts the conservative initialization into a smaller operating radius without sacrificing coverage.

The qualitative panels in Figures~\ref{fig:quadswarm-qual} and~\ref{fig:quadswarm-qual-baselines} support this interpretation. As the robust radius contracts, the ego trajectory straightens and the tubes around representative environment agents shrink accordingly, yet they continue to cover the realized trajectories. By contrast, the baseline trajectories look visually similar in the early episodes precisely because the homogeneous interaction response is mild; the important difference is not a dramatic trajectory change, but the persistent gap in how much safety margin each method carries.

\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/Fig_1_Radius_across_episodes.eps}
    \caption{Radius}\label{fig:radius}
  \end{subfigure}\hspace{10pt}%
  \begin{subfigure}[t]{0.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/Fig_3_Performance_across_episodes.eps}
    \caption{Performance}\label{fig:perf}
  \end{subfigure}\\[5pt]
  \begin{subfigure}[t]{0.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/Fig_7_Empirical_tube_coverage.eps}
    \caption{Tube cov.}\label{fig:tube}
  \end{subfigure}\hspace{10pt}%
  \begin{subfigure}[t]{0.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/Fig_6_Empirical_safety_coverage.eps}
    \caption{Safety cov.}\label{fig:safety}
  \end{subfigure}
  \caption{Two-dimensional car--pedestrian case study. Top left: evolution of the planning radius $r_j$ over episodes. Top right: evolution of the optimal cost $J_j$. Bottom left: empirical tube coverage $\mathbb{P}\{y_{j,0:T}\in \mathcal{C}_{r_j}(\hat y_{0:T})\}$. Bottom right: empirical safety coverage $\mathbb{P}\{H(x_{j,0:T},y_{j,0:T})\le 0\}$.}
  \label{fig:convergence}
\end{figure}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.35\linewidth]{figure/1}
%     \includegraphics[width=0.36\linewidth]{figure/2}\\
%     \includegraphics[width=0.35\linewidth]{figure/3}
%     \includegraphics[width=0.35\linewidth]{figure/4}
%     \caption{Two-dimensional car--pedestrian case study. Top left: evolution of the planning radius $r_j$ over episodes. Top right: evolution of the optimal cost $J_j$. Bottom left: empirical tube coverage $\mathbb{P}\{y_{j,0:T}\in \mathcal{C}_{r_j}(\hat y_{0:T})\}$. Bottom right: empirical safety coverage $\mathbb{P}\{H(x_{j,0:T},y_{j,0:T})\le 0\}$.}
%     \label{eq:results}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \subfigure[Radius]{\includegraphics[width=0.35\linewidth]{figure/Fig_1_Radius_across_episodes.eps}\label{fig:radius}}
%   \hspace{10pt}
%   \subfigure[Performance]{\includegraphics[width=0.35\linewidth]{figure/Fig_3_Performance_across_episodes.eps}\label{fig:perf}}
%   \\[5pt]
%   \subfigure[Tube cov.]{\includegraphics[width=0.35\linewidth]{figure/Fig_7_Empirical_tube_coverage.eps}\label{fig:tube}}
%   \hspace{10pt}
%   \subfigure[Safety cov.]{\includegraphics[width=0.35\linewidth]{figure/Fig_6_Empirical_safety_coverage.eps}\label{fig:safety}}
%   \caption{2D car-pedestrian example. ...}
%   \label{fig:convergence}
% \end{figure}

\begin{figure}[!tbp]
    \centering
    \captionsetup{font=small,skip=2pt}

    \begin{subfigure}[t]{0.24\linewidth}
        \centering\small $(a_1)$\\[-0.1em]
        \includegraphics[width=\linewidth]{radius_across_episodes}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.24\linewidth}
        \centering\small $(a_2)$\\[-0.1em]
        \includegraphics[width=\linewidth]{performance_cumulative_reward}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.24\linewidth}
        \centering\small $(a_3)$\\[-0.1em]
        \includegraphics[width=\linewidth]{tube_coverage}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.24\linewidth}
        \centering\small $(a_4)$\\[-0.1em]
        \includegraphics[width=\linewidth]{empirical_safety_coverage}
    \end{subfigure}

    \caption{Homogeneous QuadSwarm quantitative results. Left to right: deployed radius $r_j$ (with the currently measured quantile overlaid for the robust method), cumulative reward, empirical tube coverage, and empirical safety coverage. The key observation is that all methods remain safe in this mild homogeneous regime, but the proposed robust update sheds the most conservatism and therefore achieves the best reward.}
    \label{fig:quadswarm-metrics}
\end{figure}

\begin{figure*}[!tbp]
    \centering
    \captionsetup{font=small,skip=2pt}
    \setlength{\tabcolsep}{0pt}
    \renewcommand{\arraystretch}{0.0}

    \begin{tabular}{@{}ccccc@{}}
        \includegraphics[width=0.20\linewidth]{robust/trajectories_episode_1} &
        \includegraphics[width=0.20\linewidth]{robust/trajectories_episode_2} &
        \includegraphics[width=0.20\linewidth]{robust/trajectories_episode_3} &
        \includegraphics[width=0.20\linewidth]{robust/trajectories_episode_4} &
        \includegraphics[width=0.20\linewidth]{robust/trajectories_episode_5}
    \end{tabular}

    \vspace{-0.55em}

    \begin{tabular}{@{}ccccc@{}}
        \includegraphics[width=0.20\linewidth]{robust/agent_0/tube_1} &
        \includegraphics[width=0.20\linewidth]{robust/agent_0/tube_2} &
        \includegraphics[width=0.20\linewidth]{robust/agent_0/tube_3} &
        \includegraphics[width=0.20\linewidth]{robust/agent_0/tube_4} &
        \includegraphics[width=0.20\linewidth]{robust/agent_0/tube_5}
    \end{tabular}

    \vspace{-0.55em}

    \begin{tabular}{@{}ccccc@{}}
        \includegraphics[width=0.20\linewidth]{robust/agent_2/tube_1} &
        \includegraphics[width=0.20\linewidth]{robust/agent_2/tube_2} &
        \includegraphics[width=0.20\linewidth]{robust/agent_2/tube_3} &
        \includegraphics[width=0.20\linewidth]{robust/agent_2/tube_4} &
        \includegraphics[width=0.20\linewidth]{robust/agent_2/tube_5}
    \end{tabular}

    \caption{Qualitative evolution of the proposed robust method across episodes $j=1$--$5$ (left to right). Row~1 shows realized trajectories (solid) together with the nominal predicted trajectories used for tube construction (dotted). Rows~2 and~3 show conformal tubes for two representative environment agents. The shrinking radius allows a less conservative ego path while the tubes continue to cover the realized environment motion.}
    \label{fig:quadswarm-qual}
\end{figure*}

\begin{figure}[!tbp]
    \centering
    \captionsetup{font=small,skip=2pt}
    \setlength{\tabcolsep}{0pt}
    \renewcommand{\arraystretch}{0.0}

    \begin{tabular}{@{}ccccc@{}}
        \multicolumn{2}{c}{Na{\"i}ve} &
        \multicolumn{2}{c}{Calibrate-once} &
        Non-interactive \\

        \includegraphics[width=0.19\linewidth]{naive/trajectories_episode_1} &
        \includegraphics[width=0.19\linewidth]{naive/trajectories_episode_2} &
        \includegraphics[width=0.19\linewidth]{cal_once/trajectories_episode_1} &
        \includegraphics[width=0.19\linewidth]{cal_once/trajectories_episode_1001} &
        \includegraphics[width=0.19\linewidth]{non_int/trajectories_episode_1} \\[-0.55em]

        \includegraphics[width=0.19\linewidth]{naive/agent_0/tube_1} &
        \includegraphics[width=0.19\linewidth]{naive/agent_0/tube_2} &
        \includegraphics[width=0.19\linewidth]{cal_once/agent_0/tube_1} &
        \includegraphics[width=0.19\linewidth]{cal_once/agent_0/tube_1001} &
        \includegraphics[width=0.19\linewidth]{non_int/agent_0/tube_1} \\[-0.55em]

        \includegraphics[width=0.19\linewidth]{naive/agent_2/tube_1} &
        \includegraphics[width=0.19\linewidth]{naive/agent_2/tube_2} &
        \includegraphics[width=0.19\linewidth]{cal_once/agent_2/tube_1} &
        \includegraphics[width=0.19\linewidth]{cal_once/agent_2/tube_1001} &
        \includegraphics[width=0.19\linewidth]{non_int/agent_2/tube_1}
    \end{tabular}

    \caption{Qualitative baseline comparison. The naive baseline is shown at episodes $j=1$ and $j=2$; the calibrate-once baseline is shown at episodes $j=1$ and $j=1001$; and the non-interactive baseline is shown at episode $j=1$. In this homogeneous regime the trajectories look similar, so the main difference is the amount of tube inflation each method carries rather than a dramatic change in the environment response.}
    \label{fig:quadswarm-qual-baselines}
\end{figure}



% -----------------------------------------------------------------------------
% Quadswarm experiment section (compact, cross-referenced to main.tex)
% -----------------------------------------------------------------------------


